Unification of Quantum Graph Properties

Many properties of classical graphs are defined in terms of subsets of the vertex set. Examples include connected components, which are subsets $X \subseteq V(G)$ such that $X \times X^c$ and $E(G)$ are disjoint, or independent sets, for which $X \times X$ and $E(G)$ are disjoint. Direct generalisations of these definitions to quantum graphs are difficult to achieve, since the natural notion of subsets of a quantum set is much too rigid. As a consequence, approaches to generalising these classical properties to the quantum setting have been eclectic. In some cases, multiple inequivalent definitions of the same notion are in use. We introduce a natural and well-motivated alternative definition of subsets of a quantum set. Building on this, we propose unified definitions of quantum graph properties as straightforward generalisations of the classical definitions. We recover this way the established notions of colourings and connected components. For independent sets and cliques, our approach suggests variations that diverge from existing definitions, but address some of their counterintuitive properties. We nevertheless show how to recover an important existing definition of independent sets in our framework.

==> style/shapes.tex <==
\makeatletter
\pgfkeys{/pgf/apex angle/.initial=110}

\pgfdeclareshape{cut triangle up}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       
        
        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt - \shift}{\pgf@ya+\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{\pgf@xa-\shift}{-\pgf@ya+\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth-\shift}{-\pgf@ya+\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth-\shift}{\yintersect+\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}

\pgfdeclareshape{cut triangle down}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \savedanchor\textsize{
        \pgf@x=.5\wd\pgfnodeparttextbox
        \pgf@y=.5\ht\pgfnodeparttextbox
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       

        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt - \shift}{-\pgf@ya-\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{\pgf@xa - \shift}{\pgf@ya-\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth - \shift}{\pgf@ya-\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth - \shift}{-\yintersect-\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}

\pgfdeclareshape{cut triangle up alt}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       
        
        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt + \shift}{\pgf@ya+\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{-\pgf@xa+\shift}{-\pgf@ya+\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth+\shift}{-\pgf@ya+\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth+\shift}{\yintersect+\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}

\pgfdeclareshape{cut triangle down alt}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \savedanchor\textsize{
        \pgf@x=.5\wd\pgfnodeparttextbox
        \pgf@y=.5\ht\pgfnodeparttextbox
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       

        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt + \shift}{-\pgf@ya-\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \shift}{\pgf@ya-\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth + \shift}{\pgf@ya-\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth + \shift}{-\yintersect-\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}
\makeatother

